Learning Staged Trees from Incomplete Data

Staged trees are probabilistic graphical models capable of representing any class of non-symmetric independence via a coloring of its vertices. Several structural learning routines have been defined and implemented to learn staged trees from data, under the frequentist or Bayesian paradigm. They assume a data set has been observed fully and, in practice, observations with missing entries are either dropped or imputed before learning the model. Here, we introduce the first algorithms for staged trees that handle missingness within the learning of the model. To this end, we characterize the likelihood of staged tree models in the presence of missing data and discuss pseudo-likelihoods that approximate it. A structural expectation-maximization algorithm estimating the model directly from the full likelihood is also implemented and evaluated. A computational experiment showcases the performance of the novel learning algorithms, demonstrating that it is feasible to account for different missingness patterns when learning staged trees.

==> comp.tex <==
\begin{tikzpicture}
\renewcommand{\xx}{2.3}
\renewcommand{\yy}{0.7}
\node (v1) at (0*\xx,0*\yy) {\stage{white}{0}};
\node (v2) at (1*\xx,1.5*\yy) {\stage{white}{1}};
\node (v3) at (1*\xx,-1.5*\yy) {\stage{white}{2}};
\node (v4) at (2*\xx,3*\yy) {\stage{white}{3}};
\node (v5) at (2*\xx,1*\yy) {\stage{white}{4}};
\node (v6) at (2*\xx,-1*\yy) {\leaf};
\node (v7) at (2*\xx,-3*\yy) {\leaf};
\node (l1) at (3*\xx,3.5*\yy) {\leaf};
\node (l2) at (3*\xx,2.5*\yy) {\leaf};
\node (l3) at (3*\xx,1.5*\yy) {\leaf};
\node (l4) at (3*\xx,0.5*\yy) {\leaf};
\draw[->] (v1) -- node [above, sloped] {\scriptsize{ICU  = No}} (v2);
\draw[->] (v1) -- node [below, sloped] {\scriptsize{ICU = Yes}} (v3);
\draw[->] (v2) --  node [above, sloped] {\scriptsize{INT = No}} (v4);
\draw[->] (v2) -- node [below, sloped] {\scriptsize{INT = Yes}} (v5);
\draw[->] (v3) -- node [above, sloped] {\scriptsize{D = No}} (v6);
\draw[->] (v3) -- node [below, sloped] {\scriptsize{D = Yes}} (v7);
\draw[->] (v4) -- node [above, sloped] {\scriptsize{D = No}} (l1);
\draw[->] (v4) -- node [below, sloped] {\scriptsize{D = Yes}} (l2);
\draw[->] (v5) -- node [above, sloped] {\scriptsize{D = No}} (l3);
\draw[->] (v5) -- node [below, sloped] {\scriptsize{D = Yes}} (l4);
\end{tikzpicture}

==> xor.tex <==
\begin{tikzpicture}
\renewcommand{\xx}{2.3}
\renewcommand{\yy}{0.7}
\node (v1) at (0*\xx,0*\yy) {\stage{white}{0}};
\node (v2) at (1*\xx,1.5*\yy) {\stage{cyan}{1}};
\node (v3) at (1*\xx,-1.5*\yy) {\stage{orange}{2}};
\node (v4) at (2*\xx,3*\yy) {\stage{yellow}{3}};
\node (v5) at (2*\xx,1*\yy) {\stage{orange}{4}};
\node (v6) at (2*\xx,-1*\yy) {\leaf};
\node (v7) at (2*\xx,-3*\yy) {\leaf};
\node (l1) at (3*\xx,3.5*\yy) {\leaf};
\node (l2) at (3*\xx,2.5*\yy) {\leaf};
\node (l3) at (3*\xx,1.5*\yy) {\leaf};
\node (l4) at (3*\xx,0.5*\yy) {\leaf};
\draw[->] (v1) -- node [above, sloped] {\scriptsize{ICU  = No}} (v2);
\draw[->] (v1) -- node [below, sloped] {\scriptsize{ICU = Yes}} (v3);
\draw[->] (v2) --  node [above, sloped] {\scriptsize{INT = No}} (v4);
\draw[->] (v2) -- node [below, sloped] {\scriptsize{INT = Yes}} (v5);
\draw[->] (v3) -- node [above, sloped] {\scriptsize{D = No}} (v6);
\draw[->] (v3) -- node [below, sloped] {\scriptsize{D = Yes}} (v7);
\draw[->] (v4) -- node [above, sloped] {\scriptsize{D = No}} (l1);
\draw[->] (v4) -- node [below, sloped] {\scriptsize{D = Yes}} (l2);
\draw[->] (v5) -- node [above, sloped] {\scriptsize{D = No}} (l3);
\draw[->] (v5) -- node [below, sloped] {\scriptsize{D = Yes}} (l4);
\end{tikzpicture}
